Generating Sequences by Learning to Self-Correct

Sequence generation applications require satisfying semantic constraints, such as ensuring that programs are correct, using certain keywords, or avoiding undesirable content. Language models, whether fine-tuned or prompted with few-shot demonstrations, frequently violate these constraints, and lack a mechanism to iteratively revise their outputs. Moreover, some powerful language models are of extreme scale or inaccessible, making it inefficient, if not infeasible, to update their parameters for task-specific adaptation. We present Self-Correction, an approach that decouples an imperfect base generator (an off-the-shelf language model or supervised sequence-to-sequence model) from a separate corrector that learns to iteratively correct imperfect generations. To train the corrector, we propose an online training procedure that can use either scalar or natural language feedback on intermediate imperfect generations. We show that Self-Correction improves upon the base generator in three diverse generation tasks - mathematical program synthesis, lexically-constrained generation, and toxicity control - even when the corrector is much smaller than the base generator.

==> figures/algorithm_learning.tex <==
\newcommand{\algcomment}[1]{{\footnotesize \fontfamily{cmtt}\selectfont // #1}}
d\renewcommand{\algorithmiccomment}[1]{\hfill{\(\triangleright\)~#1}\par}
\begin{figure}[t]
\begin{algorithm}[H]
\small
\begin{algorithmic}[1]
\INPUT{Initial generator $p_0$, prompts $X$, value $V(\cdot)$,
KL weight $\beta$, number of \partitions $K$}
%
\STATE \texttt{Initialize} data pool $\mathcal{D}$ \algorithmiccomment{Initialization}
%
\FOR{iteration $= 1, 2, \ldots, N$}
\FOR{$x_i \in X$} 
\STATE \text{Sample generation $y_i \sim$ } $p_\theta(\cdot|x_i,r_{K})$ \algorithmiccomment{Exploration}
\STATE Add $\big(x_i, y_i, r(x_i, y_i)\big)$ into data pool $\mathcal{D}$
\ENDFOR
\STATE $\tilde{\mathcal{D}}_i \leftarrow$\texttt{quantize}$(\mathcal{D}; K)$ \algorithmiccomment{Quantization}
\FOR{step $= 1, 2, \ldots, M$ }
\STATE Draw a batch of data $\big\{(x_i,y_i,r_{ki})\big\}$ from quantized data pool $\tilde{\mathcal{D}}_i$ \algorithmiccomment{Learning}
\STATE Compute the objectives in Eq. \ref{eqn:learning}
\STATE Update the policy parameters $\theta$ via gradient descent
\ENDFOR
\ENDFOR
%
\end{algorithmic}
%
\caption{\methodname (\methodnameshort)}
\label{alg:main}
\end{algorithm}
\end{figure}

==> tables/commongen-e2e.tex <==

% \begin{table*}[t!]
%     \centering\footnotesize
%     \begin{tabular}{lcccccccc}
%     \toprule
%          & \textbf{Rouge} & \textbf{Bleu-4} & \textbf{CIDER} & \textbf{Constraints} & \textbf{Runtime}\\
%          \midrule
%          GPT-2~[\citenum{}]        & 40.30 & 24.70 & 13.40 & 82.20 & 0.2s/sent\\
%          NeuroLogic~[\citenum{}]         & 42.80 & 26.7 & 14.70 & 97.70& 2.04s/sent\\
%          NeuroLogic-A*esque~[\citenum{}]      & 43.60 & 28.2 & 15.20 & 97.80   & 19.24s/sent\\
%          \midrule
%          GPT-2       &  & 27.90 & 14.97 & 91.38 & 0.2s/sent\\
%          \textsc{Self-Correct} & 53.06 & 27.98 & 15.30 & 94.58 & 0.8s/sent\\
%          \textsc{Self-Correct}+NeuroLogic & 53.21 & 28.17 & 15.28 & \textbf{97.80} & 2.24s/sent\\
%     \bottomrule
%     \end{tabular}
%     \caption{Evaluation results of lexically-constrained generation on \textsc{CommonGen}. 
%     GPT-2 is the initial generator for \textsc{Self-Correct}.
%     % Runtime is estimated based on \citep{} \fb{Ximing let me know how you computed runtime.}.
%     }
%     \label{tab:toxicity_results}
% \end{table*}


\begin{table*}[t!]
\setlength\tabcolsep{3.5pt}
\renewcommand{\arraystretch}{1.2}
    \centering\scriptsize
    \begin{tabular}{l|cccc|cccccc|c}
    \toprule
    & \multicolumn{4}{c|}{\textbf{CommonGen}} & \multicolumn{6}{c|}{\textbf{E2E}} & \\ 
       \textbf{Model} & \textbf{Cov.} & \textbf{R-L} & \textbf{B-4} & \textbf{CID.}  &  \textbf{Cov.} &  \textbf{B-4} & \textbf{NIST} & \textbf{R-L}  & \textbf{MET.} & \textbf{CID.} & \textbf{Runtime}\\
        %  \midrule
        \hline \hline
        %  GPT-2~[\citenum{}]       & 82.20 & 40.30 & 24.70 & 13.40  & & & & & & & 0.2s/sent\\
         NeuroLogic~[\citenum{}]      & 97.70   & 42.80 & 26.7 & 14.70 & & & & & & & 2.04s/sent\\
         NeuroLogic-A*esque~[\citenum{}]    & 97.80  & 43.60 & 28.2 & 15.20 & & & & & &  & 19.24s/sent\\
         \midrule
         GPT-2     & 91.38  &  & 27.90 & 14.97  & 91.50 & 67.12 & 8.67 & 70.25  & \textbf{45.58} & 2.33 &  0.2s/sent\\
         \textsc{Self-Correct} & 94.58 & 53.06 & 27.98 & 15.30   & \textbf{98.77} & \textbf{68.81}  & 8.78 & 68.60 & 45.11 & \textbf{2.38} & 0.8s/sent\\
        %  \textsc{Self-Correct} 6k & 94.58 & 53.06 & 27.98 & 15.30   & 97.00 & 68.78  & \textbf{8.82} & \textbf{69.17} & 44.86 & 2.35 & 0.8s/sent\\

         \textsc{Self-Correct}+NeuroLogic & \textbf{97.80} & 53.21 & 28.17 & 15.28  & & & & & & & 2.24s/sent\\
    \bottomrule
    \end{tabular}
    \caption{Evaluation results of lexically-constrained generation on \textsc{CommonGen} and E2E. 
    GPT-2 is the initial generator for \textsc{Self-Correct}. \fb{In case we want a unified table. TODO Ximing.}
    % Runtime is estimated based on \citep{} \fb{Ximing let me know how you computed runtime.}.
    }
    \label{tab:commongen_e2e}
\end{table*}

==> tables/commongen_qual.tex <==

\begin{table}[]
\footnotesize
\setlength\tabcolsep{2.0pt}
\renewcommand{\arraystretch}{1.2}

% \begin{tabular}{cllc}
% \hline
% \multicolumn{4}{c}{\textbf{CommonGen}}                                                                                                                                                              \\ \hline
% \multicolumn{1}{l|}{Constraints ($x$)}                                  & Model        & Output ($y$)                                                                                     & Value ($\phi$) \\ \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{\thead{table, paper \\ read}}}              & GPT-2        & A man is reading book on a table                                                               & 0.66        \\ \cline{2-4} 
% \multicolumn{1}{c|}{}                                                 & \corr &                                                                                                &             \\
% \multicolumn{1}{c|}{}                                                 & 1            & A man is reading a book on a table and writing on a piece of paper.                            & 1.0         \\ \hline
% \multicolumn{1}{l|}{\multirow{3}{*}{\thead{tomato, board \\ chef, piece, cut}}} & GPT-2        & A chef cuts a piece of pizza from pizza board.                                                 & 0.8         \\ \cline{2-4} 
% \multicolumn{1}{l|}{}                                                 & \corr &                                                                                                &             \\
% \multicolumn{1}{l|}{}                                                 & 1            & A chef cutting a piece of pizza on a board with tomatoes on it                                 & 1.0         \\ \hline
% \multicolumn{1}{l|}{\multirow{4}{*}{\thead{side, continue \\ jump, end, flip}}} & GPT-2        & A man is flipping a coin to continue the game                                                  & 0.4         \\ \cline{2-4} 
% \multicolumn{1}{l|}{}                                                 & \corr &                                                                                                &             \\
% \multicolumn{1}{l|}{}                                                 & 1            & He flips the bird and ends the jump with a side kick.                                          & 0.8         \\
% \multicolumn{1}{l|}{}                                                 & 2            & \thead[l]{He continues to flip the bird and he jumps over the end of the platform, \\ ending his side kick.} & 1.0         \\ \hline
% \end{tabular}


\begin{tabular}{cllc}
\hline
\multicolumn{4}{c}{\textbf{CommonGen}}                                                                                                                                                              \\ \hline
\multicolumn{1}{l|}{\textbf{Constraints} ($x$)}                                  & \multicolumn{1}{l|}{\textbf{Model}}        & \textbf{Output} ($y$)                                                                                     & \textbf{Value} ($\phi$) \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{\thead{table, paper \\ read}}}              & \multicolumn{1}{l|}{GPT-2}        & A man is reading book on a table                                                               & 0.66        \\ \cline{2-4} 
\multicolumn{1}{c|}{}                                                 & \multicolumn{1}{l|}{\corr} &                                                                                                &             \\
\multicolumn{1}{c|}{}                                                 & \multicolumn{1}{l|}{1}           & A man is reading a book on a table and writing on a piece of paper.                            & 1.0         \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{\thead{tomato, board \\ chef, piece, cut}}} & \multicolumn{1}{l|}{GPT-2}        & A chef cuts a piece of pizza from pizza board.                                                 & 0.8         \\ \cline{2-4} 
\multicolumn{1}{l|}{}                                                 & \multicolumn{1}{l|}{\corr} &                                                                                                &             \\
\multicolumn{1}{l|}{}                                                 & \multicolumn{1}{l|}{1}             & A chef cutting a piece of pizza on a board with tomatoes on it                                 & 1.0         \\ \hline
\multicolumn{1}{l|}{\multirow{4}{*}{\thead{side, continue \\ jump, end, flip}}} & \multicolumn{1}{l|}{GPT-2}        & A man is flipping a coin to continue the game                                                  & 0.4         \\ \cline{2-4} 
\multicolumn{1}{l|}{}                                                 & \multicolumn{1}{l|}{\corr} &                                                                                                &             \\
\multicolumn{1}{l|}{}                                                 & \multicolumn{1}{l|}{1}             & He flips the bird and ends the jump with a side kick.                                          & 0.8         \\
\multicolumn{1}{l|}{}                                                 & \multicolumn{1}{l|}{2}             & \thead[l]{He continues to flip the bird and he jumps over the end of \\ the platform, ending his side kick.} & 1.0         \\ \hline
\end{tabular}

\caption{Generation examples of initial GPT-2 and multiple \corr iterations on \textsc{CommonGen} \fb{still needs work!} \fb{I put 3 examples but we can remove some.}.
% Runtime is estimated based on \citep{} \fb{Ximing let me know how you computed runtime.}.
}
\label{tab:qual-ex-commongen}
    
\end{table}

==> tables/math_feedback.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.5\linewidth]{images/feedback_iterations.png}
\vspace{-1em}
\caption{Math: multiple corrections.}
\label{fig:math-feedback-apx}
\end{figure}

==> tables/math_feedback_multiple_corrections.tex <==
\begin{table}[t!]
    \centering\footnotesize
    \begin{tabular}{ccccccccc}
    \toprule
    \textbf{Correction} & \textbf{Correct} & \textbf{Correct*}\\
    \midrule
    0 & 49.02 & 49.02 \\
    1 & 75.10 & 75.69 \\
    2 & 80.78 & 81.57 \\
    3 & 82.16 & 82.75 \\
    \midrule
    No-feedback & 74.31 & 79.80\\
    \bottomrule
    \end{tabular}
    \caption{Effect of multiple correction iterations on program synthesis (Multitask dataset, Neo 1.5B corrector and initial generator).
    \texttt{Correct} measures correctness only on the given correction iteration, while \texttt{Correct*} measures whether any of the correction iterations so far is correct.
    }
    \label{tab:multiple-corrections}
\end{table}

==> tables/math_gpt3.tex <==

% \begin{table*}[t!]
%     \centering\footnotesize
%     \begin{tabular}{llcccc}
%     \toprule
%          \textbf{Dataset} & \textbf{Generator} & \textbf{Params} & \textbf{Correct} & \textbf{+\textsc{Self-Correct}}& \textbf{+\textsc{Self-Correct}$_*$}\\
%          \midrule
%          \textbf{Multiarith} & GPT-3 Curie & 6B & 43.3 & \textbf{97.5} & \textbf{97.5}\\
%          & GPT-3 Davinci & 175B&                  68.3 & \textbf{95.0} & \textbf{97.5}\\
%          & GPT-3 Text-Davinci-002 & 175B&         92.5 & \textbf{95.8} & \textbf{100.0}\\
%          % & \textit{GPT-Neo} & \textit{1.3B} & \textit{60.00} & \textit{98.33} & \textit{99.17}\\
%          \midrule
%          \textbf{Multitask}  & GPT-3 Curie & 6B & 30.0 & \textbf{71.6} & \textbf{75.4}\\
%          & GPT-3 Davinci &175B& 46.7 & \textbf{72.8} & \textbf{80.0}\\
%          & GPT-3 Text-Davinci-002 & 175B & 84.9 & 73.6 & \textbf{90.9}\\
%          \midrule
%          \textbf{GSM8k} & GPT-3 Curie & 6B & 2.01 & \textbf{20.60} & \textbf{21.10}\\
%          & GPT-3 Davinci & 175B & 6.96 & \textbf{21.00} & \textbf{24.30}\\
%          & GPT-3 Text-Davinci-002 & 175B & 36.8 & 21.10 & \textbf{45.00}\\
%     \bottomrule
%     \end{tabular}
%     \caption{Generalizing to correcting larger models that differ from the generator used in training. As the correction model we use GPT-Neo 1.3B from our previous experiments trained with a GPT-Neo 1.3B initial generator. 
%     GPT-3 models use 10-shot prompts (5 for GSM8k due to context length).
%     % As a reference we show the correction model's performance with the GPT-Neo 1.3B initial generator used in training. 
%     }
%     \label{tab:math_gpt3_results}
% \end{table*}

\begin{table*}[t!]
    \centering\footnotesize
    \begin{tabular}{lllcccc}
    \toprule
         \textbf{Dataset} & \textbf{Generator (train)} & \textbf{Generator (test)} & \textbf{Generator} & \textbf{Self-corrector}\\
         \midrule
         Multitask %& Neo 1.3B & Neo 1.3B & 49.02 & 78.24\\
                            & Neo 1.3B & GPT-3 & 46.70 & 80.00\\
                            & Neo 1.3B & GPT-3 Instruct & 84.90 & 90.90\\
                            & GPT-3 Instruct  & GPT-3 Instruct & 84.90 & 92.75\\
         \midrule
         GSM %& Neo 1.3B & Neo 1.3B & 8.60 & 23.96  \\
                        & Neo 1.3B & GPT-3  & 6.96 & 24.30 \\
                        & Neo 1.3B & GPT-3 Instruct  & 36.80 & 45.00\\
                        & GPT-3 Instruct  & GPT-3 Instruct  & 36.80 & 45.92\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Modularity (program synthesis).} Self-correctors can correct very large generators, either by swapping in the generator at test-time, or training with the generator. The corrector is GPT-Neo 1.3B, and here we only correct incorrect outputs.
    GPT-3 and GPT-3 Instruct refer to the \texttt{davinci} and \texttt{text-davinci-002} engines on the OpenAI API, respectively.
    }
    \label{tab:math_gpt3_results}
\end{table*}

==> tables/math_iterative.tex <==
\begin{table}[t!]
    \centering\footnotesize
    \begin{tabular}{ccccccccc}
    \toprule
    \textbf{Training} & \textbf{Multiarith} & \textbf{Multitask} & \textbf{GSM8k}\\
    \midrule
    Non-iterative & 89.20 & 73.49 & 17.60 \\
    Iterative & \textbf{99.17} & \textbf{78.24} & \textbf{23.96}\\
    \bottomrule
    \end{tabular}
    \caption{Effect of iterative training on program synthesis (Neo 1.5B corrector and initial generator).
    }
    \label{tab:multiple-corrections}
\end{table}

==> tables/math_valid.tex <==

\begin{table*}[t!]
    \centering\footnotesize
    \begin{tabular}{llccc}
    \toprule
         \textbf{Dataset} & \textbf{Model} & \textbf{Params} & \textbf{Correct}\\
         \midrule
         \textbf{Multiarith} & GPT-NEO & 1.3B & 60.00\\
         & +\textsc{Self-Correct} & 1.3B & \textbf{98.33}\\
         & +$\textsc{Self-Correct}_*$ & 1.3B & \textbf{99.17}\\
         \midrule
         \textbf{Multitask} %&GPT-NEO~[\citenum{mishra2022lila}] & 2.7B & 59.70\\
         %\cmidrule(lr){2-4}
         & GPT-NEO & 1.3B & 49.02\\
         & +\textsc{Self-Correct} & 1.3B & \textbf{73.33}\\
         & +$\textsc{Self-Correct}_*$ & 1.3B & \textbf{77.84}\\
         \midrule
         \textbf{GSM8k} 
         & \textit{OpenAI 3B}~[\citenum{cobbe2021gsm8k}] & 3B& 15.50\\
         & \textit{OpenAI 6B}~[\citenum{cobbe2021gsm8k}] & 6B\citenum{}& 20.00\\
         & GPT-NEO~[\citenum{ni2022learning}] & 2.7B\citenum{}& 18.80\\
         & NEO FCP+PCP~[\citenum{ni2022learning}] & 2.7B\citenum{}& 19.50\\
         % & \textit{GPT-3}~[\citenum{cobbe2021gsm8k}] & 12B\citenum{}& 23.00\\
         \cmidrule(lr){2-4}
         & GPT-NEO & 1.3B & 8.57\\
         & +\textsc{Self-Correct} & 1.3B & \textbf{21.15}\\
         & +$\textsc{Self-Correct}_*$ & 1.3B & \textbf{23.96}\\
         % +feedback\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Validation set}. Evaluation results of mathematical program synthesis experiments. GPT-NEO (1.3B) is the initial generator for \textsc{Self-Correct}. 
    $\textsc{Self-Correct}_*$ refers to the oracle inference setting.
    \textit{(Italicized)}: original non-program variant of GSM8k. All models (including baselines) are finetuned.
    }
    \label{tab:math_results}
\end{table*}


==> tables/modularity_both.tex <==

\begin{table}[t]
\begin{minipage}[t]{0.54\linewidth}
\centering\footnotesize
\setlength{\tabcolsep}{4pt}
% \renewcommand\arraystretch{1.14}
   \begin{tabular}{lccc}
    \toprule
         \textbf{Test Generator} & \textbf{Correct$_*$} & \textbf{Fluency} & \textbf{Constraints} \\
         \midrule
         NeuroLogic~[\citenum{lu-etal-2021-neurologic}] &  2.04s & 14.70 & 97.70\\
         NeuroLogic-A*~[\citenum{lu2022neurologicastar}]& 19.24s & 15.20 & 97.80 \\
         \midrule
         GPT-2 & 0.20s & 14.97 & 91.38 \\
         \method & 0.80s& 15.30 & 94.58 \\
         \ \ +NeuroLogic & 2.24s& 15.28 & \textbf{97.80} \\
    \bottomrule
    \end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\linewidth}
\centering \footnotesize
% \renewcommand\arraystretch{1.2}
    \begin{tabular}{lllcccc}
    \toprule
         \textbf{Dataset} & \textbf{Generator (train)} & \textbf{Generator (test)} & \textbf{Generator} & \textbf{Self-corrector}\\
         \midrule
         Multitask %& Neo 1.3B & Neo 1.3B & 49.02 & 78.24\\
                            & GPT-3 & 46.70 & 80.00\\
                            & GPT-3 Instruct & 84.90 & 90.90\\
                            &\ \ +train & 84.90 & 92.75\\
         \midrule
         GSM %& Neo 1.3B & Neo 1.3B & 8.60 & 23.96  \\
                        & GPT-3  & 6.96 & 24.30 \\
                        & GPT-3 Instruct  & 36.80 & 45.00\\
                        &\ \ +train  & 36.80 & 45.92\\
    \bottomrule
    \end{tabular}
    % \caption{\textbf{Modularity (program synthesis).} Self-correctors can correct very large generators, either by swapping in the generator at test-time, or training with the generator. The corrector is GPT-Neo 1.3B, and here we only correct incorrect outputs.
    % GPT-3 and GPT-3 Instruct refer to the \texttt{davinci} and \texttt{text-davinci-002} engines on the OpenAI API, respectively. }
    \label{tab:math_gpt3_results}
\end{minipage}
\caption{\textbf{Modularity}
See the Appendix for all metrics.}
    \label{tab:lexical_results}
\end{table}

==> tables/toxicity_modularity.tex <==

\begin{table*}[t!]
    \centering\footnotesize
    \begin{tabular}{lcccccccc}
    \toprule
         & \multicolumn{2}{c}{\textbf{Toxicity $\uparrow$}}& \textbf{Fluency}& \multicolumn{2}{c}{\textbf{Diversity}}\\
         \cmidrule(lr){2-3}\cmidrule(lr){4-4}\cmidrule(lr){5-6}
         \textbf{Generator (test)} & \textbf{Avg.~Max}. & \textbf{Prob.} & \textbf{Perplexity} & \textbf{dist-2} & \textbf{dist-3} \\
         \midrule
         % GPT2-L        & 0.527 & 0.520 & 11.31 & 0.85 & 0.85 \\
         % +Self-corrector & 0.171 & 0.026 & 11.20 & 0.80 & 0.83\\
                  % \midrule
         GPT2-XL & 0.383 & 0.268 & 8.67 & 0.81 & 0.83 \\
         +\method & 0.166 & 0.022 & 11.86 &0.80 & 0.83\\
         \midrule
         %          GPT3-ada & & & & & \\
         % \textsc{Self-Correct}  & & & & & \\
         %          \midrule
         GPT3-davinci & & & & & \\
         +\method  & & & & & \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Modularity (toxicity).} 
    % Self-correctors with a large generator (GPT2-XL, GPT3) and a smaller corrector that is trained with a GPT-L generator.
    % 
    Generating initial sequences from a large generator  then refining them to have lower toxicity with a smaller corrector. 
    % The corrector refines the generator's sequences to have lower toxicity.
    The corrector is trained with a GPT-L generator.
    }
    \label{tab:toxicity_module}
\end{table*}

